Bagging is an Optimal PAC Learner

Determining the optimal sample complexity of PAC learning in the realizable setting was a central open problem in learning theory for decades. Finally, the seminal work by Hanneke (2016) gave an algorithm with a provably optimal sample complexity. His algorithm is based on a careful and structured sub-sampling of the training data and then returning a majority vote among hypotheses trained on each of the sub-samples. While being a very exciting theoretical result, it has not had much impact in practice, in part due to inefficiency, since it constructs a polynomial number of sub-samples of the training data, each of linear size. In this work, we prove the surprising result that the practical and classic heuristic bagging (a.k.a. bootstrap aggregation), due to Breiman (1996), is in fact also an optimal PAC learner. Bagging pre-dates Hanneke's algorithm by twenty years and is taught in most undergraduate machine learning courses. Moreover, we show that it only requires a logarithmic number of sub-samples to reach optimality.

==> backup.tex <==
\subsection{Proving Lemma~\ref{lem:goodG}}
What remains is thus to prove Lemma~\ref{lem:goodG}. This is the technically most challenging part of the proof. To bound $\Loss^{1/3}(g_S)$, we first show that we can ignore bootstrap samples $B \in S^n$ where $B$ has few distinct samples. Concretely, for a $B \in S^n$, let $\size(B)$ denote the number of distinct samples in $B$. Also, for any $1 \leq k \leq n$, let $S^n_k$ denote the subset of $S^n$ consisting of all $B$ with $\size(B)=k$.

We first show:
\begin{lemma}
  Assume there is a universal constant $c > 0$ such that for every $0 < \gamma < 1$ and every $k$ with $(\rho/2)n \leq k \leq \min\{n, (1-1/e)m\}$, it holds with probability at least $1-\gamma$ over a set of $m$ samples $S \sim \Dist^m$ that
  \[
    \Loss^{1/12}_\Dist(g_{S_k}) \leq c \cdot \frac{d + \ln(1/\gamma)}{m},
  \]
  then it holds with probability at least $1-7\gamma$ over $S \sim \Dist^m$ that
  \[
    \Loss^{1/3}_\Dist(g_S) \leq 8c \cdot \frac{d + \ln(1/\gamma)}{m}.
  \]
\end{lemma}
\begin{proof}
  Let $\chi_S^{1/3}(x)$ take the value $1$ if $\Pr_{\boot \sim S^n}[h_\boot(x) \neq c(x)] > 1/3$ and $0$ otherwise. Similarly, let $\chi^{1/12}_{S,k}(x)$ take the value $1$ if $\Pr_{\boot \sim S^n_k}[h_\boot(x) \neq c(x)] > 1/12$ and $0$ otherwise. Notice that if $\chi_S^{1/3}(x)=1$ then we must have $\sum_{k=1}^n \Pr_{\boot \sim S^n}[\size(\boot)=k] \Pr_{\boot \sim S^n_k}[ h_\boot(x) \neq c(x)] > 1/3$. Using that $\Pr_{\boot \sim S^n_k}[ h_\boot(x) \neq c(x)] \leq \chi^{1/12}_{S,k}(x) + 1/12$ it must hold that $\sum_{k=1}^n \Pr_{\boot \sim S^n}[\size(\boot)=k] \chi^{1/12}_{S,k}(x) \geq 1/3-1/12 = 1/4$. Thus we have:
  \[
    \chi^{1/3}_S(x) \leq 4 \sum_{k=1}^n \Pr_{\boot \sim S^n}[\size(\boot)=k] \chi^{1/12}_{S,k}(x).
  \]
  In particular, this implies that $\E_{x \sim \Dist(\cdot \mid \chi^{1/3}_S(x)=1)}[\sum_{k=1}^n \Pr_{\boot \sim S^n}[\size(\boot)=k] \chi^{1/12}_{S,k}(x)] \geq 1/4$ which further implies $\sum_{k=1}^n \Pr_{\boot \sim S^n}[\size(\boot)=k] \E_{x \sim \Dist(\cdot \mid \chi^{1/3}_S(x)=1)}[\chi^{1/12}_{S,k}(x)] \geq 1/4$. If let $Z$ be the random variable that with probability $\Pr_{\boot \sim S^n}[\size(\boot)=k]$ takes the value $\E_{x \sim \Dist(\cdot \mid \chi^{1/3}_S(x)=1)}[\chi^{1/12}_{S,k}(x)]$, then this is $\E[Z] \geq 1/4$. Moreover, since $Z$ takes values of at most $1$, we may consider the non-negative variable $1-Z$. This variable has expectation at most $3/4$. Hence by Markov's inequality, we have $\Pr[Z \leq 1/8] = \Pr[1-Z \geq 7/8] \leq (3/4)/(7/8) = 6/7$. Thus $\sum_{k : \E_{x \sim \Dist(\cdot \mid \chi^{1/3}_S(x)=1)}[\chi^{1/12}_{S,k}(x)] > 1/8} \Pr_{\boot \sim S^n}[\size(\boot)=k] \geq 1/7$. Next observe that if $ \E_{x \sim \Dist(\cdot \mid \chi^{1/3}_S(x)=1)}[\chi^{1/12}_{S,k}(x)] > 1/8$ then $\Pr_{x \sim \Dist}[\chi^{1/12}_{S,k}(x)=1] \geq \Pr_{x \sim \Dist}[\chi^{1/3}_S(x)=1]/8$. We hence conclude that if $S$ satisfies $\Loss^{1/3}_\Dist(g_S) > 8c \cdot \frac{d + \ln(1/\gamma)}{m}$ then $\sum_{k : \Loss^{1/12}_{\Dist}(g_{S_k}) > c (d + \ln(1/\gamma))/m} \Pr_{\boot \sim S^n}[\size(\boot)=k] \geq 1/7$. Thus
  \[
    \Pr_{S \sim \Dist^m} [\Loss^{1/3}_\Dist(g_S) > 8c \cdot \frac{d + \ln(1/\gamma)}{m}] \leq \Pr_{S \sim \Dist^m}[\sum_{k : \Loss^{1/12}_{\Dist}(g_{S_k}) > c (d + \ln(1/\gamma))/m} \Pr_{\boot \sim S^n}[\size(\boot)=k] \geq 1/7 ]
  \]
  Let $\kappa$ take the value $k$ with probability $\Pr_{\boot \sim S^n}[\size(\boot)=\kappa]$ and let $Y_{S,\kappa}$ taking the value $1$ if $\Loss^{1/12}_{\Dist}(g_{S_\kappa}) > c (d + \ln(1/\gamma))/m$ and $0$ otherwise. Then the above is
  \begin{eqnarray*}
    \Pr_{S \sim \Dist^m} [\Loss^{1/3}_\Dist(g_S) > 8c \cdot \frac{d + \ln(1/\gamma)}{m}] &\leq& \Pr_{S \sim \Dist^m}[\E_\kappa[Y_{S,\kappa}] \geq 1/7 ] \\
                                                                                         &\leq& 7 \cdot \E_{S \sim \Dist^m}[\E_\kappa[Y_{S,\kappa}]] \\
                                                                                         &=&  7 \cdot \E_\kappa[\E_{S \sim \Dist^m}[ Y_{S,\kappa}]] \\
                                                                                         &\leq& 7 \cdot \max_k \E_{S \sim \Dist^m}[ Y_{S,k}] \\
                                                                                         &=& 7 \cdot \max_k \Pr_{S \sim \Dist^m}[\Loss^{1/12}_{\Dist}(g_{S_k}) > c (d + \ln(1/\gamma))/m ] \\
    &\leq& 7 \gamma. 
  \end{eqnarray*}
\end{proof}

define a family $\Fam = \{\Buc_1,\Buc_2,\dots,\Buc_N \}$. Each $\Buc_i \in \Fam$ is a collection of $m/2$-sized subsets of $[m] = \{1,\dots,m\}$. The family $\Fam$ has the property that every $A_i \in \binom{[m]}{m/2}$ occurs in equally many collections $\Buc_j$, and every $\Buc_j$ has the same cardinality. For every $A_i \in \binom{[m]}{m/2}$, we naturally associate a subset $S_i \in \binom{S}{m/2}$, corresponding to picking out the samples in $S$ indexed by $A_i$. With a slight abuse of notation, let $h(A_i) = h(S_i)$, where $S_i$ is the associated subset of $S$.

These properties imply that an $h_i$ drawn uniformly from $\Gs(S)$, has the same distribution as an $h_i$ obtained by first drawing a uniform random $\Buc_j$, and then a uniform random $A_k$ in $\Buc_j$ and letting $h_i = h(A_k)$. To exploit this, let $X(S,\Buc_j,x)$ be an indicator taking the value $1$ if $|\{A_i \in \Buc_j : (h(A_i))(x) \neq c(x) \}| > |\Buc_j|/6$. Then:
\begin{lemma}
  \label{lem:buckets}
For every $S$, if we let $\Buc_j$ be uniform in $\Fam$, then it holds that $\Loss^{1/3}_\Dist(\Gs(S)) \leq 6\cdot \Pr_{\Buc_j ,x \sim \Dist}[X(S,\Buc_j,x)=1]$.
\end{lemma}
\begin{proof}
  Fix an $S$. Let $x \in \Xs$ be such that $| \{ h \in \Gs(S) : h(x) \neq c(x) \}| > |\Gs(S)|/3$. For such $x$, if we first draw a uniform $\Buc_j$ and then a uniform $A_i$ in $\Buc_j$, then $\Pr_{\Buc_j,A_i}[(h(A_i))(x) \neq c(x)] \geq 1/3$. But
  \begin{eqnarray*}
    \Pr_{\Buc_j,A_i}[(h(A_i))(x) \neq c(x)] &=& \Pr_{\Buc_j}[X(S,\Buc_j,x)=1]  \Pr_{A_i}[(h(A_i))(x) \neq c(x) \mid X(S,\Buc_j,x)=1] \\
                                            &+& \Pr_{\Buc_j}[X(S,\Buc_j,x)=0]  \Pr_{A_i}[(h(A_i))(x) \neq c(x) \mid X(S,\Buc_j,x)=0] \\
    &\leq& \Pr_{\Buc_j}[X(S,\Buc_j,x)=1] + 1/6.
  \end{eqnarray*}
  Hence $1/3 \leq \Pr_{\Buc_j}[X(S,\Buc_j,x)=1] + 1/6 \Rightarrow \Pr_{\Buc_j}[X(S,\Buc_j,x)=1] \geq 1/6$. It follows by linearity that $\Pr_{\Buc_j ,x \sim \Dist}[X(S,\Buc_j,x)=1] \geq \Loss^{1/3}_\Dist(\Gs(S))/6$.
\end{proof}
By Lemma~\ref{lem:buckets}, it thus suffices to carefully define the family $\Fam$ such that with probability $1-\delta$ over $S$, we have $\Pr_{\Buc_j ,x \sim \Dist}[X(S,\Buc_j,x)=1] \leq c'(d + \ln(1/\delta))/m$ for a constant $c'>0$.

To define $\Fam$, we take some inspiration from Hanneke's PAC learning algorithm with optimal sample complexity in the realizable case. Let $C = 13$. Let $\beta = \lfloor \lg_C(m/2) \rfloor$. We define a collection $\Buc_j = \Buc(I)$ for every list $I=(i_1,\dots,i_{C^\beta})$ of $C^\beta$ distinct indices in $[m]$. A set $A \in \binom{[m]}{m/2}$ is included in $\Buc(I)$ if and only if the following holds:
\begin{itemize}
\item For every $j=1,\dots,\beta$, let $I_j$ denote the first $C^j$ indices in $I$. Partition these indices into $C$ groups of $C^{j-1}$ indices, such that the first group $G_1$ has the first $C^{j-1}$ indices, $G_2$ has the next $C^{j-1}$ indices and so forth. Among the groups $G_2,\dots,G_C$, there is precisely one group $G_i$ such that $A$ has none of the indices in $G_i$, and for the remaining groups $G_i$ among $G_2,\dots,G_C$, $A$ has all the indices in $G_i$.
\end{itemize}
Symmetry implies that each $A$ is included in equally many collections $\Buc_j$. Similarly, each $\Buc_j$ has equally many sets $A$. Furthermore, $\Buc_j \neq \emptyset$ since the requirement to be in $\Buc_j$ forces $C^\beta - \sum_{j=0}^{\beta - 1} C^{j} < m/2$ indices to be included in $A$ and $\sum_{j=0}^{\beta- 1} C^j < m/2$ indices to be excluded.

With this definition, we show the following for all $\Buc_j$:
\begin{lemma}
  \label{lem:goodBuckets}
  There is a universal constant $c'>0$, such that for every collection $\Buc_j \in \Fam$ and every $0 < \delta < 1$, it holds with probability at least $1-\delta$ over $S$, that $\Pr_{x \sim \Dist}[X(S,\Buc_j,x)=1] \leq c'(d + \ln(1/\delta))/m$.
\end{lemma}
Before proving Lemma~\ref{lem:goodBuckets}, let us see that it suffices to complete the proof of Lemma~\ref{lem:goodG} and thus of Theorem~\ref{thm:main}.

\begin{proof}[Proof of Lemma~\ref{lem:goodG}]
  Fix a $0 < \delta < 1$ as in Lemma~\ref{lem:goodG}. Let $N$ be the number of collections $\Buc_j$ in $\Fam$. Define for each $\Buc_j \in \Fam$ and every integer $i \geq 0$ the indicator $B_{i,j}(S)$ taking the value $1$ if
  \[
    \Pr_{x \sim \Dist}[X(S,\Buc_j,x)=1] \in (2^ic'(d + \ln(8/\delta))/m, 2^{i+1}c'(d + \ln(8/\delta))/m].
  \]
  If we let $\Buc_j$ be uniform random in $\Fam$, then for a fixed $S$, we have:
  \begin{eqnarray*}
    \Pr_{\Buc_j, x \sim \Dist}[X(S,\Buc_j,x)=1] &\leq& \sum_{i=0}^\infty 2^{i+1} c'(d + \ln(8/\delta))/m \cdot \frac{\sum_{j=1}^N B_{i,j}(S)}{N}
  \end{eqnarray*}
  Now call an $S$ \emph{good} if, for all integers $i \geq 0$, it holds that $\frac{\sum_{j=1}^N B_{i,j}(S)}{N} \leq 4^{-i}$. For good $S$, the above implies
\begin{eqnarray*}
  \Pr_{\Buc_j, x \sim \Dist}[X(S,\Buc_j,x)=1] &\leq& \sum_{i=0}^\infty 2^{i+1} c'(d + \ln(8/\delta))/m \cdot 4^{-i} \\
  &\leq& 4 c'(d + \ln(8/\delta))/m.
\end{eqnarray*}
By Lemma~\ref{lem:buckets}, it follows that for \emph{good} $S$, we have $\Loss^{1/3}(\Gs(S)) \leq 24 \cdot c'(d + \ln(8/\delta))/m \leq c(d + \ln(1/\delta))/m$ for big enough constant $c>0$. Thus what remains is to show that $S$ is good with probability at least $1-\delta$. To prove this, let $F_i$ denote the event that  $\sum_{j=1}^N B_{i,j}(S) > 4^{-i}N$. We need to show that $\sum_{i=0}^\infty \Pr[F_i] \leq \delta$. For this, we use Markov's inequality to conclude that $\Pr[F_i] \leq (4^i/N) \cdot \sum_{j=1}^N \Pr_S[B_{i,j}(S)=1]$. Since $2^ic'(d + \ln(8/\delta))/m \geq c'(d + \ln((8/\delta)^{2^i}))/m$, it follows from Lemma~\ref{lem:goodBuckets} that $\Pr_S[B_{i,j}(S)=1] \leq (\delta/8)^{2^i}$. We thus have $\Pr[F_i] \leq (4^i/N) \cdot N (\delta/8)^{2^i} = 4^i (\delta/8)^{2^i} < \delta 2^{-(i+1)}$. We thus conclude that $\sum_{i=0}^\infty \Pr[F_i] \leq \sum_{i=0}^\infty \delta 2^{-(i+1)} = \delta$, completing the proof of Lemma~\ref{lem:goodG}.
\end{proof}

\subsection{Proving Lemma~\ref{lem:goodBuckets}}
We have now reduced the task to proving Lemma~\ref{lem:goodBuckets}, i.e. showing that for every $0 < \delta < 1$ and any collection $\Buc_j \in \Fam$, it holds with probability at least $1-\delta$ over $S$, that $\Pr_{x \sim \Dist}[X(S,\Buc_j,x)=1] \leq c'(d + \ln(1/\delta))/m$. Recall that each $\Buc_j$ is defined from a list of indices $I$. We will switch to refering to $\Buc_j$ as $\Buc_I$ instead. To simplify notation a bit, we will write $\Loss^{1/6}_\Dist(\Buc_I):=\Pr_{x \sim \Dist}[X(S,\Buc_I,x)=1] = \Pr_{x \sim \Dist}[|\{A_i \in \Buc_I : (h(A_i))(x) \neq c(x) \}| > |\Buc_I|/6]$.

To bound $\Loss^{1/6}_\Dist(\Buc_I)$, we first define a tree $\Tree$. The tree $\Tree$ is a $(C-1) = 12$-ary tree with $\beta+1$ levels. Each node $v \in \Tree$ has an associated subset $\Asso^v \subseteq \Buc_j$. For a node $v$, we use the notation $\Asso^v_i$ to denote the subset associated with the $i$'th child of $v$, i.e. if node $w$ is the $i$'th child of $v$, then $\Asso^v_i = \Asso^w$. For notational convenience, we index the children of a node $v$ from $i=2$ to $i=C$. We assign the sets $A \in \Buc_I$ to the nodes of $\Tree$, by assigning each $A$ to every node along a root-to-leaf path. The path traversed for a subset $A$ is defined as follows: Call the level of the root $\beta$ and the level of the leaves $0$. Start by assigning $A$ to the root node at level $\beta$. Then, in each step, if $A$ is currently at a node $v$ in level $j > 0$, let $I_j$ denote the first $C^j$ indices in the list of indices $I$ defining $\Buc_I$. Recall the partitioning of these indices into groups $G_1,\dots,G_C$ and recall that for any $A$, there is precisely one of the groups $G_i$ among $G_2,\dots,G_C$ for which $A$ contains no indices. Moreover, $A$ contains every index in every other group $G_i$ among $G_2,\dots,G_C$. If $i \in \{2,\dots,C\}$ denotes the group for which $A$ contains no indices, then we recursively assign $A$ to the $i$'th child of $v$.

Consider a node $v \in \Tree$ and define $\Loss^{1/6}_\Dist(\Asso^v) := \Pr_{x \sim \Dist}[|\{A \in \Asso^v : (h(A))(x) \neq c(x)\} |> |\Asso^v|/6]$. Then for the root node $r$, it holds that $\Loss_\Dist^{1/6}(\Asso^r) = \Loss_\Dist^{1/6}(\Buc_I)$. We will prove by induction that for every $0 < \delta < 1$, and for every node $v$ in level $j$, it holds with probability at least $1-\delta$ over $S$ that
\[
  \Loss_\Dist^{1/6}(\Asso^v) \leq c'' \cdot \frac{d + \ln(1/\delta)}{C^j}
\]
for a universal constant $c'' > 0$. Since the root $r$ is at level $j = \beta = \lfloor \lg_C(m/2) \rfloor$, this implies $\Loss_\Dist^{1/6}(\Buc_I) =\Loss_\Dist^{1/6}(\Asso^r) \leq c'(d + \ln(1/\delta))/m$ with probability at least $1-\delta$ over $S$ (where $c'>0$ is a constant).

The base case $j=0$ is trivial as the claim follows immediately by noting that $c'' d/C^0 \geq 1$. For the inductive step, consider some level $j > 0$, a value of $\delta$ between $0$ and $1$, and some node $v$ in that level. Again, if $c''(d + \ln(1/\delta))/C^j \geq 1$ then the claim follows trivially. Thus assume $c''(d + \ln(1/\delta))/C^j < 1$. By the induction hypothesis, it holds for every $0 < \delta' < 1$ and every child $i \in \{2,\dots,C\}$ of $v$, that $\Loss_\Dist^{1/6}(\Asso^v_i) \leq c'' (d + \ln(1/\delta'))/C^{j-1}$ with probability at least $1-\delta'$ over $S$.

For each child $i$ of $v$, define an event $E_i$ that occurs if $\Loss_\Dist^{1/6}(\Asso^v_i) > c'' (d + \ln((3C)/\delta))/C^{j-1}$. Then $\Pr_S[E_i] \leq \delta/(3C)$ by induction.

Consider next a child $i$ and any set $\bar{A} \in \Asso^v$ that is assigned to a child $k \neq i$. Let $h = h(\bar{A})$ denote the hypothesis obtained from $\bar{A}$. We seek to bound
\[
  \Pr_{x \sim \Dist}[|\{A \in \Asso^v_i : (h(A))(x) \neq c(x)\} |> |\Asso^v_i|/6 \wedge h(x) \neq c(x)].
\]
That is, we want to show that it is unlikely that at least a $1/6$-fraction of the hypotheses obtained from $\Asso^v_i$ mispredict the label of an $x$ \emph{at the same time} as $h$ mispredicts the label. The intuitive reason for why this is true, is that $h$ is trained on all the samples corresponding to indices in group $G_i$ while all sets $A \in \Asso^v_i$ excludes all those samples. For notational convenience, let $S^v_i \subseteq S$ denote the samples $(x_\ell, c(x_\ell))$ with $\ell \in G_i$. Also, let $\Err_i \subseteq \Xs$ denote the set of $x \in \Xs$ for which $|\{A \in \Asso^v_i : (h(A))(x) \neq c(x)\} |> |\Asso^v_i|/6$.

We now define the event $E'_i$ that occurs if both of the following hold:
\begin{enumerate}
\item $\Loss^{1/6}_\Dist(\Asso^v_i) \geq (c''/1000)(d + \ln(1/\delta))/C^j$.
\item $|S^v_i \cap \Err_i| < c''(d + \ln(1/\delta))/(2000 C)$ (if $S^v_i$ is a multi-set, the intersection preserves duplicates).
\end{enumerate}
We start by bounding $\Pr[E'_i]$. For this, we simply bound the probability that the second condition holds conditioned on the first. Notice that since all $A \in \Asso^v_i$ exclude all samples from $S^v_i$, we have that the samples $(x,c(x)) \in S^v_i$ are independent of $\{h(A) : A \in \Asso^v_i\}$. Thus if $\Loss^{1/6}_\Dist(\Asso^v_i) \geq (c''/1000)(d + \ln(1/\delta))/C^j$, we expect to see at least $\mu := C^{j-1}(c''/10)(d + \ln(1/\delta))/C^j = c''(d + \ln(1/\delta))/(1000C)$ samples $(x, c(x))$ for which $|\{A \in \Asso^v : (h(A))(x) \neq c(x)\} |> |\Asso^v|/6$. If $c''$ is sufficiently large compared to $C=13$, then $\mu \geq 8 \ln((3C)/\delta)$. In that case, a Chernoff bound implies that we see less than $\mu/2$ such samples with probability at most $\exp(-(1/2)^2\mu/2) \leq \exp(-\ln((3C)/\delta)) = \delta/(3C)$. We conclude $\Pr[E'_i] \leq \delta/(3C)$.

The final event we need to define, denoted $E''_i$, occurs when both of the following hold:
\begin{enumerate}
\item $|S^v_i \cap \Err_i| \geq c''(d + \ln(1/\delta))/(2000C)$.
\item There is a hypothesis $h \in \Hyp$ with $h(x) = c(x)$ for all $(x, c(x)) \in (S^v_i \cap \Err_i)$, but $\Loss_{\Dist(\cdot \mid \Err_i)}(h) > 1/(1000 C)$.
\end{enumerate}
We bound $\Pr[E''_i]$ by bounding the probability that the second condition holds conditioned on the first. For this, observe that if we condition on the set of indices of the samples $(x,c(x))$ in $S^v_i \cap \Err_i$, then these samples are i.i.d. from the distribution $\Dist(\cdot \mid \Err_i)$, i.e. from the distribution $\Dist$ conditioned on $x \in \Err_i$. Classic generalization bounds for the realizable setting shows that with probability at least $1-\delta/(3C)$ over $m$ samples $S'$ from \emph{any} distribution $\Dist'$, it holds that \emph{every} hypothesis $h \in \Hyp$ with $h(x) = c(x)$ for all $(x,c(x)) \in S'$ satisfy $\Loss_{\Dist'}(h) \leq c''' (d \ln(m/d) + \ln((3C)/\delta))/m$ for a universal constant $c'''>0$. Applying this to the distribution $\Dist' = \Dist(\cdot \mid \Err_i)$ and the samples in $S^v_i \cap \Err_i$ shows that with probability at least $1-\delta/(3C)$, it holds for every $h \in \Hyp$ with $h(x) = c(x)$ for all $(x,c(x)) \in (S^v_i \cap \Err_i)$ that:
\begin{eqnarray*}
  \Loss_{\Dist(\cdot \mid \Err_i)}(h) &\leq& c''' \cdot \frac{d \ln(|S^v_i \cap \Err_i|/d) + \ln((3C)/\delta)}{|S^v_i \cap \Err_i|}
\end{eqnarray*}
If we fix $c''$ large enough, this is decreasing for $|S^v_i \cap \Err_i| \geq c''(d + \ln(1/\delta))/(2000C)$. Since we condition on this event, we get
\begin{eqnarray*}
  \Loss_{\Dist(\cdot \mid \Err_i)}(h) &\leq& 2000C c''' \cdot \frac{d \ln(c''(d + \ln(1/\delta))/(2000Cd)) + \ln((3C)/\delta)}{c''(d + \ln(1/\delta))}
\end{eqnarray*}
If $c''$ is large enough compared to $C=13$ and $c'''$, this is at most $1/(1000 C)$ as desired. Hence $\Pr[E''_i] \leq \delta/(3C)$.

A union bound now implies that $\Pr_S[\bigcup_{i} \{E_i \cup E'_i \cup E''_i \}] \leq \delta$. Thus with probability $1-\delta$, none of the events $E_i, E'_i$ and $E''_i$ occur for any $i$. So assume henceforth that this is case and consider any child $i$ and any set $\bar{A} \in \Asso^v$ that is assigned to a child $k \neq i$. Let $h = h(\bar{A})$ denote the hypothesis obtained from $\bar{A}$. Since we run empirical risk minimization to obtain $h$, we know that $h$ correctly predicts the label of every sample it is trained on. Moreover, we know that $\bar{A}$ includes all samples from $S^v_i$. We want to prove that
\begin{eqnarray}
  \label{eq:small}
  \Pr_{x \sim \Dist}[|\{A \in \Asso^v_i : (h(A))(x) \neq c(x)\} |> |\Asso^v_i|/6 \wedge h(x) \neq c(x)] \leq (c''/1000)(d + \ln(1/\delta))/C^j.
\end{eqnarray}
We know that $E'_i$ does not occur. There are now two cases. In the first case, we have $\Loss^{1/6}_\Dist(\Asso^v_i) < (c''/1000)(d + \ln(1/\delta))/C^j$. The conclusion follows trivially:
\begin{eqnarray*}
  \Pr_{x \sim \Dist}[|\{A \in \Asso^v_i : (h(A))(x) \neq c(x)\} |> |\Asso^v_i|/6 \wedge h(x) \neq c(x)] &\leq& \\
  \Pr_{x \sim \Dist}[|\{A \in \Asso^v_i : (h(A))(x) \neq c(x)\} |> |\Asso^v_i|/6] &=& \\
  \Loss^{1/6}_\Dist(\Asso^v_i) &<& (c''/1000)(d + \ln(1/\delta))/C^j.
\end{eqnarray*}
In the second case, we have $\Loss^{1/6}_\Dist(\Asso^v_i) \geq (c''/1000)(d + \ln(1/\delta))/C^j$. Here we use that we also know that $E_i$ does not occur. Hence we also have $\Loss^{1/6}_\Dist(\Asso^v_i) \leq c''(d + \ln(1/\delta))/C^{j-1}$. Since $E'_i$ does not occur, we must have $|S^v_i \cap \Err_i| \geq c''(d + \ln(1/\delta))/(2000C)$. Since $E''_i$ does not occur, this implies that $h$ must satisfy $\Loss_{\Dist(\cdot \mid \Err_i)}(h) \leq 1/(1000 C)$. We then have
\begin{eqnarray*}
  \Pr_{x \sim \Dist}[|\{A \in \Asso^v_i : (h(A))(x) \neq c(x)\} |> |\Asso^v_i|/6 \wedge h(x) \neq c(x)] &=& \\
  \Loss^{1/6}_\Dist(\Asso^v_i) \cdot \Loss_{\Dist(\cdot \mid \Err_i)}(h) &\leq& \\
  (c''(d + \ln(1/\delta))/C^{j-1}) \cdot (1/(1000 C)).
\end{eqnarray*}
We have thus establishes Eq.~\eqref{eq:small}. What remains is to use Eq.~\eqref{eq:small} to conclude that $\Loss_\Dist^{1/6}(\Asso^v) \leq c''(d + \ln(1/\delta))/C^j$, which would complete the inductive step. Define $\Err$ as those $x \in \Xs$ for which $|\{A \in \Asso^v : (h(A))(x) \neq c(x)\}| > |\Asso^v|/6$. On any such $x$, consider drawing two sets $A_1,A_2$ uniformly and independently from $\Asso^v$. Let $h_1 = h(A_1)$ and $h_2=h(A_2)$. Since each set $\Asso^v_i$ contains equally many sets $A$, we have that $A_1$ and $A_2$ have the same distribution as if we first pick a random child $i$ among the $C-1=12$ children, and then a random $A$ from $\Asso^v_i$. Let $i_1$ denote the index of the child containing $A_1$ and let $i_2$ denote the index of the child containing $A_2$.

We first observe that there must be a child index $z(x)$ for which $|\{A \in \Asso_z^v : (h(A))(x) \neq c(x)\}| > |\Asso_z^v|/6$. Fix such a $z=z(x)$ for every $x \in \Err$ and define $z(x) =0$ for all other $x$. Even in the case that $|\{A \in \Asso_z^v : (h(A))(x) \neq c(x)\}| = |\Asso_z^v|$, there still must be another $|\Asso^v|/6 - |\Asso^v_z| = |\Asso^v|/6 - |\Asso^v|/(C-1) \geq |\Asso^v|/12$ sets $A$ in $\Asso^v \setminus \Asso^v_z$ for which $(h(A))(x) \neq c(x)$. We then have for $x \in \Err$ that:
\begin{eqnarray*}
  \Pr_{A_1,A_2}[i_1 = z \wedge i_2 \neq z \wedge h_2(x) \neq c(x)] &\geq& (1/(C-1)) \cdot (1/12) = 1/144.
\end{eqnarray*}
It follows that
\[
  \Pr_{A_1,A_2, x \sim \Dist}[i_1 = z(x) \wedge i_2 \neq z(x) \wedge h_2(x) \neq c(x)] \geq \Pr_{x \sim \Dist}[x \in \Err]/144.
\]
By averaging, there must exist a fixed choice of $A^*_1$ and $A^*_2$ such that
\[
  \Pr_{x \sim \Dist}[i^*_1 = z(x) \wedge i^*_2 \neq z(x) \wedge h_2(x) \neq c(x)] \geq \Pr_{x \sim \Dist}[x \in \Err]/144.
\]
If $i^*_1 = i^*_2$, then the left hand side is $0$ and we conclude $\Loss_\Dist^{1/6}(\Asso^v) = \Pr_{x \sim \Dist}[x \in \Err] = 0$. Otherwise, we have $i^*_1 \neq i^*_2$. We see that
\begin{eqnarray*}
  \Pr_{x \sim \Dist}[i^*_1 = z(x) \wedge i^*_2 \neq z(x) \wedge h_2(x) \neq c(x)]  &\leq& \Pr_{x \sim \Dist}[i^*_1 = z(x) \wedge h_2(x) \neq c(x)] 
\end{eqnarray*}
Since $A^*_2$ is assigned to a child $i^*_2 \neq i^*_1$, it follows from Eq.~\eqref{eq:small} that
\begin{eqnarray*}
  \Pr_{x \sim \Dist}[i^*_1 = z(x) \wedge h_2(x) \neq c(x)] &\leq& (c''/1000)(d + \ln(1/\delta))/C^j.
\end{eqnarray*}
This finally implies
\[
  \Loss^{1/6}_\Dist(\Asso^v) = \Pr_{x \sim \Dist}[x \in \Err] \leq 144 (c''/1000)(d + \ln(1/\delta))/C^j < c''(d + \ln(1/\delta))/C^j.
\]
